EconAgentic in DePIN Markets: A Large Language Model Approach to the Sharing Economy of Decentralized Physical Infrastructure

The Decentralized Physical Infrastructure (DePIN) market is revolutionizing the sharing economy through token-based economics and smart contracts that govern decentralized operations. By 2024, DePIN projects have exceeded \$10 billion in market capitalization, underscoring their rapid growth. However, the unregulated nature of these markets, coupled with the autonomous deployment of AI agents in smart contracts, introduces risks such as inefficiencies and potential misalignment with human values. To address these concerns, we introduce EconAgentic, a Large Language Model (LLM)-powered framework designed to mitigate these challenges. Our research focuses on three key areas: 1) modeling the dynamic evolution of DePIN markets, 2) evaluating stakeholders' actions and their economic impacts, and 3) analyzing macroeconomic indicators to align market outcomes with societal goals. Through EconAgentic, we simulate how AI agents respond to token incentives, invest in infrastructure, and adapt to market conditions, comparing AI-driven decisions with human heuristic benchmarks. Our results show that EconAgentic provides valuable insights into the efficiency, inclusion, and stability of DePIN markets, contributing to both academic understanding and practical improvements in the design and governance of decentralized, tokenized economies.

==> figs/depin.tex <==
\begin{figure*}[!htbp]
\centering
\begin{tikzpicture}[
    node distance=1cm and 0.5cm,
    line/.style={draw, thick, -Latex},
    arrowText/.style={midway, fill=white, font=\footnotesize, align=center},
    depin/.style={rectangle, draw, fill=blue!20, text width=5cm, align=center, rounded corners, minimum height=1cm, font=\footnotesize},
    cepin/.style={rectangle, draw, fill=red!20, text width=5cm, align=center, rounded corners, minimum height=1cm, font=\footnotesize},
    title/.style={font=\bfseries, align=center, text width=7cm}
]

% Titles
\node[title, anchor=west] (cepinTitle) at (0,0) {(CePIN) Centralized \\Physical Infrastructure };
\node[title, anchor=east] (depinTitle) at (16,0) {(DePIN) Decentralized \\ Physical Infrastructure Networks };

% Nodes for CePIN
\node[cepin, below=1cm of cepinTitle.west, anchor=west] (capexC) {High capital expenditure, centralized equipment};
\node[cepin, below=of capexC.west, anchor=west] (laborC) {Labor-intensive, professional installation};
\node[cepin, below=of laborC.west, anchor=west] (maintC) {High maintenance and operational costs};
\node[cepin, below=of maintC.west, anchor=west] (realC) {Significant real estate costs};
\node[cepin, below=of realC.west, anchor=west] (marketC) {Constrained by local monopolies};

% Nodes for DePIN
\node[depin, below=1cm of depinTitle.east, anchor=east] (capexD) {Lower capital expenditure, crowdsourced hardware};
\node[depin, below=of capexD.east, anchor=east] (laborD) {Simplified, DIY installation};
\node[depin, below=of laborD.east, anchor=east] (maintD) {Reduced maintenance costs, decentralized operations};
\node[depin, below=of maintD.east, anchor=east] (realD) {Reduced real estate and operational expenses};
\node[depin, below=of realD.east, anchor=east] (marketD) {Open and global market access};

% Connecting lines
\draw[line] (capexC.east) -- (capexD.west) node[arrowText] {\$ \textbf{Capital Expenditure}};
\draw[line] (laborC.east) -- (laborD.west) node[arrowText] {\ding{72} \textbf{Labor Costs}};
\draw[line] (maintC.east) -- (maintD.west) node[arrowText] {\ding{42} \textbf{Maintenance and Operation}};
\draw[line] (realC.east) -- (realD.west) node[arrowText] {\ding{73} \textbf{Real Estate and Operational Expenses}};
\draw[line] (marketC.east) -- (marketD.west) node[arrowText] {\ding{115} \textbf{Market Access and Coverage}};

\end{tikzpicture}
\caption{Comparative analysis of Centralized (CePIN) vs. Decentralized (DePIN) Physical Infrastructure Networks, highlighting the economic and operational differences.}
\label{fig:depin}
\end{figure*}
